MCU-MixQ: A HW/SW Co-optimized Mixed-precision Neural Network Design Framework for MCUs

Mixed-precision neural network (MPNN) that utilizes just enough data width for the neural network processing is an effective approach to meet the stringent resources constraints including memory and computing of MCUs. Nevertheless, there is still a lack of sub-byte and mixed-precision SIMD operations in MCU-class ISA and the limited computing capability of MCUs remains underutilized, which further aggravates the computing bound encountered in neural network processing. As a result, the benefits of MPNNs cannot be fully unleashed. In this work, we propose to pack multiple low-bitwidth arithmetic operations within a single instruction multiple data (SIMD) instructions in typical MCUs, and then develop an efficient convolution operator by exploring both the data parallelism and computing parallelism in convolution along with the proposed SIMD packing. Finally, we further leverage Neural Architecture Search (NAS) to build a HW/SW co-designed MPNN design framework, namely MCU-MixQ. This framework can optimize both the MPNN quantization and MPNN implementation efficiency, striking an optimized balance between neural network performance and accuracy. According to our experiment results, MCU-MixQ achieves 2.1$\times$ and 1.4$\times$ speedup over CMix-NN and MCUNet respectively under the same resource constraints.

==> sections/section5.tex <==
%\def\inlinecode#1{\texttt{#1}}
%\section{SIMD-aware Mixed-Precision Quantization}
% Previous work\cite{cai2020rethinking, DQSS, DNAS, Edd, OSMPS} has shown that NAS is an effective method to quantize a model. Taking the proposed SLBC kernel into consideration, we employ differentiable NAS to search for the optimal composition of bitwidth for a model architecture. 
% % However, prior work seem to ignore complexity related to hardware. 
% % TODO: FLOPs can't be proxy
% However, most prior works target FLOPs as the proxy to estimate model latency, which ignores the impact of memory access on model performance, thus failing to reflect the model performance on MCU devices accurately. Especially for MPNN which involves diverse bit-widths, memory access will lead to a greater impact on inference latency. \par
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% To tackle this problem, we combine quantization search stage with it. During the search phase, each kernel to be quantized can be regarded as a mixture of multiple kernels of the same kind, each of which equips with a weight coefficient. \par
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Distinct from naïve convolution, which primarily involves standard MACs, the proposed SLDC method substitutes multiple SISD \inlinecode{MUL} and \inlinecode{ADD} instructions with a more efficient SIMD \inlinecode{MUL} instruction and a few of bit operations. Considering the varied execution time of diverse instructions, we use SISD instructions as the complexity calibration benchmark and align SIMD \inlinecode{MUL} instruction and SISD bit operations with it by introducing adjusting hyper-parameters. More specifically, as shown in Eq. \ref{eq:op_complexity}, the complexity of SISD instructions $C_{SISD}$ is directly proportional to the number of SISD accumulation and multiplication operations, while that of SIMD instructions and bit operations is directly proportional to the number of SIMD multiplication and bit operations respectively. What's more, to make quantization search aware of the impact of different quantization bitwidth and suppress the tendency too favor higher bitwidth in the selection process, complexity should also be inversely proportional to the memory space it occupies. As a result, %TODO
% The overall complexity $C$ is the sum of all kinds of complexity mentioned above with a adjusting super-parameter as defined in Eq. \ref{eq:total_complexity}.

% \begin{equation}
%     C=C_{SISD}+\alpha C_{SIMD}+\beta C_{bit}
% \label{eq:total_complexity}
% \end{equation}
% \begin{equation}
% \label{eq:op_complexity}
%     C_{OP}=\sum_{l}^{L}{\frac{\#ops_{l}}{\sum_{q_{w}}^{Q_{w}}{\sum_{q_{a}}^{Q_{a}}{\alpha_{q_w}\alpha_{q_a}w(q_w)a(q_a)}}}}
%     % C_{OP}=\#ops
% \end{equation}
% % TODO: complexity的表示
% % Due to the differences of execution time between diverse instructions,  Using SISD instructions as the calibration benchmark, SIMD instrucions and SISD bit operations are assigned a hyperparameter to align with it. The SIMD aware optimization objective is formulated as follows.
% Given a quantization search space $Q=\{q_1,q_2,...,q_n\}$, the quantization super-net can be denoted as $f(Q)$, while a sub-net sampled from $Q$ is $f(q_i)$. The optimization object is to seek for a quantization configuration $q^{*}$ to maximize the accuracy and minimize the latency while satisfying the constraints, SRAM and flash for example. Since the quantized kernel has been discreted, now we can use back propagation to minimize the loss.

% \begin{equation}
%     Loss(\alpha_{w}, \alpha_{a})=Loss_{acc}(\alpha_{w}, \alpha_{a})+Loss_{comp}(\alpha_{w}, \alpha_{a})
% \end{equation}
% \begin{equation}
% \label{eq:target}
%     Loss=Loss_{acc}+\eta Loss_{comp}
% \end{equation}

% Finally, for each quantized kernel, the bitwidth with highest $\alpha$ will be chosen as the ultimate kernel quantization. After quantization search stage, MCU-MixQ performs QAT(quantization aware training) on the mixed precision model and obtain a well-trained model. Next, the model will be mapped to the corresponding operators optimized for MCU, completing the entire workflow of the end to end framework.
% 2 stage quantization
